Selective Ensemble Based on Preference-Directed Multi-Objective Bandits

Selective ensemble for modern machine learning systems requires choosing promising model candidates under limited evaluation budgets, while downstream tasks often specify only partial preferences over capabilities such as accuracy, robustness, and reasoning. This setting naturally gives rise to a sequential decision problem under partially specified linear preferences. We formalize it as preference-directed multi-objective bandits (PDMOB), where admissible trade-offs are represented by a polyhedral preference cone. Based on this formulation, we introduce Pareto $C$-optimality, which recovers standard Pareto optimality and single-weight scalarization as special cases. We then propose the preference-directed upper confidence bound (PrefUCB) algorithm, which maintains directional confidence intervals to guide exploration. We analyze both indicator-based and gap-weighted regret, and establish instance-dependent logarithmic bounds for both criteria, recovering the optimal logarithmic dependence on the horizon $T$ in classical special cases. Experiments on large pre-trained model selective ensemble tasks and online asset allocation under institutional mandates validate the efficacy of our method.

==> sections/extra_experiments.tex <==
%!TEX root = ../arxiv/main.tex


\section{Online Asset Allocation}
\label{sec:experiments}

In this section, we evaluate the \texttt{PrefUCB} algorithm on the Online Asset Allocation tasks. We formulate this as a Preference-Directed Multi-Objective Bandit (PDMOB) task, where the learner must sequentially select investment strategies to satisfy specific financial mandates.

\subsection{Experimental Setup}

\paragraph{Dataset and Base Strategies}
We utilize the NYSE(O) dataset~\citep{li2014online}, comprising 36 stocks from the New York Stock Exchange over 22 years (July 1962 to December 1984)~\citep{cover1991universal}. From this data, we construct a diverse pool of $K=10$ base strategies (actions). These strategies encompass a range of investment approaches, from passive benchmarks (Uniform Buy-and-Hold) to active learning algorithms (OLMAR, CWMR) and risk-aware methods (Risk Parity).

\paragraph{Objectives and Feedback}
At each time step $t$, the learner selects a strategy and observes a 7-dimensional reward vector consisting of normalized metrics: Cumulative Wealth Growth (CWG), Sharpe Ratio (SR), Maximum Drawdown (MDD), Sortino Ratio, Alpha, Turnover (TO), and Calmar Ratio (CR).

\paragraph{Financial Mandates}
To simulate realistic institutional requirements, we define eight distinct financial ``mandates'' (e.g., Aggressive Growth, Market Neutral, Low Volatility). Each mandate is characterized by a preference matrix $W \in \mathbb{R}^{3 \times 7}$, constructed using a data-driven heuristic based on historical performance. Detailed methodologies for preference construction, along with the specific weight vectors and descriptions for each mandate, are provided in Appendix~\ref{app:mandate_details}.

\paragraph{Baselines}
We compare \texttt{PrefUCB} against the following baselines:
\begin{compactitem}
    \item \textbf{ParetoUCB}~\citep{DBLP:conf/ijcnn/DruganN13}: A standard multi-objective bandit algorithm adapted as a selective ensemble method. It selects base models according to standard Pareto optimality without accounting for preference direction.
    \item \textbf{ScalarizedUCB\(_{r.r.}\)}~\citep{DBLP:conf/ijcnn/DruganN13}: This method converts multi-objective feedback into scalar rewards by randomly selecting a row from the preference matrix as the scalarization vector.
    \item \textbf{GT-PF} (Ground Truth Pareto Front): An oracle-based benchmark that randomly selects from the true Pareto-optimal set. This represents the theoretical upper bound for preference-agnostic ensemble methods~\citep{DBLP:conf/aaai/QianYZ15} under perfect information.
\end{compactitem}

\subsection{Results and Discussion}

We report the cumulative regret after $T=5,651$ rounds, averaged over 20 independent trials. Lower regret indicates that the algorithm more frequently selected strategies satisfying the specific mandate (Pareto C-optimality).

\paragraph{Performance Analysis}
Table~\ref{tab:main_results} presents the normalized cumulative regret across the eight scenarios. \texttt{PrefUCB} demonstrates consistent superiority, particularly in mandates requiring specific directional trade-offs.

In aggressive scenarios, such as \textit{Aggressive Growth} and \textit{Momentum Concentrated}, \texttt{PrefUCB} significantly outperforms all baselines. Notably, in the \textit{Momentum Concentrated} mandate, \texttt{PrefUCB} achieves a normalized regret of 0.059 compared to 0.130 for the next best baseline (ScalarizedUCB), a 54.6\% improvement. This suggests that standard Pareto approaches struggle to distinguish risky but preferred strategies from those that are safe but irrelevant to the mandate.

For complex trade-offs, such as the \textit{Market Neutral Hedge} scenario, \texttt{PrefUCB} (0.280) reduces regret by over 40\% compared to ScalarizedUCB (0.469). This validates the algorithm's capability to navigate polyhedral cones where the optimal region constitutes a narrow segment of the Pareto front.

In defensive scenarios like \textit{High Frequency Trading} and \textit{Low Volatility}, the performance gap narrows. For \textit{High Frequency Trading}, ParetoUCB (0.806) slightly outperforms \texttt{PrefUCB} (0.808), although the difference is not statistically significant. This outcome is expected; when mandates prioritize risk minimization or balanced objectives, the preferred strategies often align with the anchor points of the global Pareto front, allowing generic multi-objective algorithms to perform adequately.

Overall, \texttt{PrefUCB} provides the most robust performance across diverse financial environments (Figure~\ref{fig:regret}), achieving the best average rank of 1.13.

\begin{table*}[h!]
\centering
\caption{Performance comparison of \textsf{PrefUCB} against baseline variants across different financial market scenarios. Reported values are the normalized cumulative regret (mean $\pm$ std) with rank in parentheses. Lower regret is better. The best performance in each scenario is highlighted in bold. Statistical significance (t-test): \CIRCLE~indicates the baseline is significantly worse than \textsf{PrefUCB} ($p < 0.05$); \Circle~indicates no significant difference. \textsf{PrefUCB} achieves the best average rank (1.13) and wins in 7 out of 8 scenarios.}
\label{tab:main_results}
\begin{minipage}{\textwidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
{Scenario} & {\textsf{PrefUCB} (Ours)} & {$\mbox{ScalarizedUCB}_{\text{r.r.}}$} & {\textsf{ParetoUCB}} & {\textsf{GTPF}} \\
\midrule
Aggressive Growth & \textbf{0.142 $\pm$ 0.004~(1)} & 0.288 $\pm$ 0.003~(2)~\CIRCLE & 0.295 $\pm$ 0.004~(3)~\CIRCLE & 0.351 $\pm$ 0.035~(4)~\CIRCLE \\
Market Neutral Hedge & \textbf{0.280 $\pm$ 0.008~(1)} & 0.469 $\pm$ 0.005~(2)~\CIRCLE & 0.679 $\pm$ 0.008~(4)~\CIRCLE & 0.601 $\pm$ 0.042~(3)~\CIRCLE \\
High Frequency Trading & 0.808 $\pm$ 0.004~(2) & 0.819 $\pm$ 0.009~(3)~\CIRCLE & \textbf{0.806 $\pm$ 0.003~(1)}~\Circle & 0.847 $\pm$ 0.028~(4)~\CIRCLE \\
Income Focused & \textbf{0.867 $\pm$ 0.007~(1)} & 0.941 $\pm$ 0.002~(3)~\CIRCLE & 0.909 $\pm$ 0.002~(2)~\CIRCLE & 0.997 $\pm$ 0.007~(4)~\CIRCLE \\
Low Volatility & \textbf{0.790 $\pm$ 0.017~(1)} & 0.815 $\pm$ 0.006~(3)~\CIRCLE & 0.806 $\pm$ 0.004~(2)~\CIRCLE & 0.848 $\pm$ 0.044~(4)~\CIRCLE \\
Momentum Concentrated & \textbf{0.059 $\pm$ 0.004~(1)} & 0.130 $\pm$ 0.002~(2)~\CIRCLE & 0.199 $\pm$ 0.003~(3)~\CIRCLE & 0.238 $\pm$ 0.052~(4)~\CIRCLE \\
Risk Parity Enhanced & \textbf{0.818 $\pm$ 0.015~(1)} & 0.862 $\pm$ 0.004~(2)~\CIRCLE & 0.899 $\pm$ 0.003~(4)~\CIRCLE & 0.864 $\pm$ 0.017~(3)~\CIRCLE \\
Balanced Growth & \textbf{0.672 $\pm$ 0.010~(1)} & 0.710 $\pm$ 0.004~(2)~\CIRCLE & 0.710 $\pm$ 0.004~(2)~\CIRCLE & 0.767 $\pm$ 0.080~(4)~\CIRCLE \\
\midrule
\midrule
\textbf{Avg. Rank} & \textbf{1.13} & 2.38 & 2.63 & 3.75 \\
\textbf{w/l/t} & --- & 0/8/0 & 1/7/0 & 0/8/0 \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\vspace{-3mm}
\end{table*}

\begin{figure*}[!t]
\begin{minipage}{.98\textwidth}
\centering
\includegraphics[width=0.98\textwidth]{./fig/cumulative_regret_8scenarios.pdf}
\end{minipage}
\vspace{-3mm}
\caption{Cumulative regret analysis across benchmark and real-world scenarios. Shaded areas represent one standard deviation.}
\label{fig:regret}
\vspace{-3mm}
\end{figure*}

\newpage
\appendix
\section{Detailed Experimental Settings and Results}
\label{app:mandate_details}

This appendix provides a comprehensive description of the preference construction methodology, the specific logic defining each financial mandate, and detailed performance visualizations.

\subsection{Data-Driven Preference Construction}

To evaluate our approach in realistic environments, we employ a rigorous data-driven heuristic to construct the preference matrix $W$ for each mandate, utilizing the historical performance of base strategies on the training partition.

\textbf{Construction Methodology.} The preference matrix $W$ is derived through a three-step procedure:
\begin{enumerate}
    \item \textbf{Metric Normalization:} All seven objective metrics are normalized to the unit interval $[0, 1]$. Objectives requiring minimization (MDD, TO) are inverted to create a unified maximization framework.
    \item \textbf{Variance-Based Priority:} For primary objectives, we assign positive weights proportional to their historical variance. This emphasizes metrics with high distinguishability.
    \item \textbf{Regression-Based Penalties:} We model trade-offs between conflicting objectives using linear regression. Negative weights are assigned to secondary objectives based on the regression coefficients ($\beta$) to penalize strategies that violate the mandate's risk tolerance.
\end{enumerate}

Each mandate is defined by a preference matrix $W \in \mathbb{R}^{3 \times 7}$, where each row $w_i$ represents an alternative weighting scheme. The algorithm evaluates strategies against all three weight vectors to capture the multi-faceted nature of institutional mandates.

\subsection{Mandate Descriptions and Weight Specifications}

We constructed $W$ for eight specific mandates. Table~\ref{tab:mandate_descriptions} details the theoretical goals and construction logic for each mandate, while Table~\ref{tab:weight_specifications} provides the exact weight vectors used in the experiments. Positive values indicate objectives to maximize, whereas negative values denote penalty terms for undesirable characteristics.

\begin{table*}[t]
\caption{Financial Mandates and Preference Logic. The weight vectors ($W$) are constructed to enforce specific trade-offs, such as penalizing volatility (negative weights) while maximizing Alpha (positive weights).}
\label{tab:mandate_descriptions}
\centering
\small
\begin{tabular}{l p{5cm} p{8cm}}
\toprule
\textbf{Mandate} & \textbf{Theoretical Goal} & \textbf{Preference Construction Logic (Excerpt)} \\
\midrule
\textbf{Aggressive Growth} & Absolute Return + Alpha + Risk Tolerance & Maximize CWG ($w \approx 0.63$) and Alpha ($w \approx 0.37$). Negative penalties applied to MDD and TO are relaxed or removed to allow aggressive positioning. \\
\midrule
\textbf{Market Neutral} & Alpha + Calmar + Downside Protection & Primary focus on Alpha ($w=1.0$) and CR. Strong negative penalties on correlation and drawdown to ensure neutrality. \\
\midrule
\textbf{High Frequency Trading} & Sharpe + Sortino + High Turnover Tolerance & Balanced emphasis on SR ($w \approx 0.50$) and Sortino ($w \approx 0.50$). Turnover penalties are removed to accommodate high-frequency rebalancing. \\
\midrule
\textbf{Income Focused} & Consistent Yield + Low Volatility & Balanced weights on CWG ($\approx 0.60$) and SR ($\approx 0.40$). Negative weights on Turnover and Alpha to discourage speculative trading. \\
\midrule
\textbf{Low Volatility} & Double Risk Control (MDD + Sortino) & Pure risk minimization: Weights distributed between MDD ($w \approx 0.72$) and Sortino ($w \approx 0.28$). Strategies with high volatility receive severe negative scores. \\
\midrule
\textbf{Momentum Conc.} & Alpha + CWG Maximization & Similar to Aggressive Growth but with higher specific weight on Alpha ($\approx 0.63$) to capture trend-following premiums. \\
\midrule
\textbf{Risk Parity Enh.} & SR + MDD Balance & Weights distributed between SR ($\approx 0.29$) and MDD ($\approx 0.71$) to enforce risk-adjusted returns over pure growth. \\
\midrule
\textbf{Balanced Growth} & Multi-Objective Equilibrium & A complex mix of CWG, SR, and Sortino, ensuring no single metric dominates. Penalties are moderate. \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Detailed Weight Specifications for Financial Mandates. Each mandate is represented by three weight vectors $w_1, w_2, w_3 \in \mathbb{R}^7$, corresponding to the seven objectives: CWG, SR, MDD, Sortino, Alpha, TO, CR.}
\label{tab:weight_specifications}
\centering
\footnotesize
\begin{tabular}{lcccccccc}
\toprule
\textbf{Mandate} & \textbf{Vector} & \textbf{CWG} & \textbf{SR} & \textbf{MDD} & \textbf{Sortino} & \textbf{Alpha} & \textbf{TO} & \textbf{CR} \\
\midrule
\multirow{3}{*}{\textbf{Aggressive Growth}}
& $w_1$ & 0.633 & 0.000 & -0.300 & 0.000 & 0.367 & 0.000 & 0.000 \\
& $w_2$ & 1.000 & 0.000 & 0.000 & -0.300 & 0.000 & -0.300 & 0.000 \\
& $w_3$ & 0.000 & 0.000 & -0.300 & 0.000 & 0.475 & -0.300 & 0.525 \\
\midrule
\multirow{3}{*}{\textbf{Market Neutral Hedge}}
& $w_1$ & 0.000 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\
& $w_2$ & -0.300 & 0.000 & 0.000 & 0.000 & 0.475 & 0.000 & 0.525 \\
& $w_3$ & 0.000 & 0.000 & 0.716 & 0.284 & 0.000 & -0.300 & 0.000 \\
\midrule
\multirow{3}{*}{\textbf{High Frequency Trading}}
& $w_1$ & 0.000 & 0.505 & 0.000 & 0.495 & 0.000 & 0.000 & 0.000 \\
& $w_2$ & 0.000 & 1.000 & -0.300 & 0.000 & -0.300 & 0.000 & 0.000 \\
& $w_3$ & 0.000 & 0.000 & 0.000 & 0.510 & 0.000 & -0.300 & 0.490 \\
\midrule
\multirow{3}{*}{\textbf{Income Focused}}
& $w_1$ & 0.595 & 0.405 & -0.300 & 0.000 & 0.000 & 0.000 & 0.000 \\
& $w_2$ & 0.000 & 0.000 & 0.000 & 1.000 & -0.300 & -0.300 & 0.000 \\
& $w_3$ & 0.000 & 0.515 & 0.000 & 0.000 & 0.000 & -0.300 & 0.485 \\
\midrule
\multirow{3}{*}{\textbf{Low Volatility}}
& $w_1$ & 0.000 & 0.000 & 0.716 & 0.284 & 0.000 & 0.000 & 0.000 \\
& $w_2$ & -0.300 & 0.000 & 0.000 & 1.000 & -0.300 & -0.300 & 0.000 \\
& $w_3$ & 0.000 & 0.287 & 0.713 & 0.000 & 0.000 & 0.000 & -0.300 \\
\midrule
\multirow{3}{*}{\textbf{Momentum Concentrated}}
& $w_1$ & 0.633 & 0.000 & 0.000 & 0.000 & 0.367 & 0.000 & 0.000 \\
& $w_2$ & 0.000 & 0.000 & -0.300 & -0.300 & 1.000 & -0.300 & 0.000 \\
& $w_3$ & 0.609 & -0.300 & 0.000 & 0.000 & 0.000 & -0.300 & 0.391 \\
\midrule
\multirow{3}{*}{\textbf{Risk Parity Enhanced}}
& $w_1$ & 0.000 & 0.287 & 0.713 & 0.000 & 0.000 & 0.000 & 0.000 \\
& $w_2$ & 0.000 & 1.000 & 0.000 & 0.000 & 0.000 & -0.300 & 0.000 \\
& $w_3$ & -0.300 & 0.000 & 0.716 & 0.284 & -0.300 & 0.000 & 0.000 \\
\midrule
\multirow{3}{*}{\textbf{Balanced Growth}}
& $w_1$ & 0.426 & 0.290 & 0.000 & 0.284 & 0.000 & 0.000 & 0.000 \\
& $w_2$ & 0.000 & 0.515 & -0.300 & 0.000 & 0.000 & -0.300 & 0.485 \\
& $w_3$ & 0.000 & 0.000 & 0.000 & 0.536 & 0.464 & -0.300 & 0.000 \\
\bottomrule
\end{tabular}
\end{table*}

\subsection{Temporal Dynamics of Objectives}

Figure~\ref{fig:sub} illustrates the temporal trends of sub-objectives across different mandates. The solid lines represent the 100-round moving average, while the shaded regions correspond to the true reward values. The results confirm that \texttt{PrefUCB} (shown in blue) consistently prioritizes preferred objectives, compromises on relaxable ones, and maintains acceptable levels for moderate objectives, demonstrating superior trade-off capabilities.

\begin{figure}[!t]
\centering
\subfigure[Aggressive Growth]{
\includegraphics[width=0.48\textwidth]{./fig/Aggressive_Growth_performance.pdf}
}
\subfigure[Market Neutral Hedge]{
\includegraphics[width=0.48\textwidth]{./fig/Market_Neutral_Hedge_performance.pdf}
}
\subfigure[High-frequency Trading]{
\includegraphics[width=0.48\textwidth]{./fig/High_Frequency_Trading_performance.pdf}
}
\subfigure[Income Focused]{
\includegraphics[width=0.48\textwidth]{./fig/Income_Focused_performance.pdf}
}
\subfigure[Low Volatility]{
\includegraphics[width=0.48\textwidth]{./fig/Low_Volatility_performance.pdf}
}
\subfigure[Momentum Concentrated]{
\includegraphics[width=0.48\textwidth]{./fig/Momentum_Concentrated_performance.pdf}
}
\subfigure[Risk Parity Enhanced]{
\includegraphics[width=0.48\textwidth]{./fig/Risk_Parity_Enhanced_performance.pdf}
}
\subfigure[Balanced Growth]{
\includegraphics[width=0.48\textwidth]{./fig/Balanced_Growth_performance.pdf}
}
\vspace{-2mm}
\caption{Temporal trends of sub-objectives across different mandate scenarios.}
\label{fig:sub}
\vspace{-4mm}
\end{figure}
